Quantum parallel information exchange (QPIE) hybrid network with transfer learning

Quantum machine learning (QML) has emerged as an innovative framework with the potential to uncover complex patterns by leveraging quantum systems ability to simulate and exploit high-dimensional latent spaces, particularly in learning tasks. Quantum neural network (QNN) frameworks are inherently sensitive to the precision of gradient calculations and the computational limitations of current quantum hardware as unitary rotations introduce overhead from complex number computations, and the quantum gate operation speed remains a bottleneck for practical implementations. In this study, we introduce quantum parallel information exchange (QPIE) hybrid network, a new non-sequential hybrid classical quantum model architecture, leveraging quantum transfer learning by feeding pre-trained parameters from classical neural networks into quantum circuits, which enables efficient pattern recognition and temporal series data prediction by utilizing non-clifford parameterized quantum gates thereby enhancing both learning efficiency and representational capacity. Additionally, we develop a dynamic gradient selection method that applies the parameter shift rule on quantum processing units (QPUs) and adjoint differentiation on GPUs. Our results demonstrate model performance exhibiting higher accuracy in ad-hoc benchmarks, lowering approximately 88% convergence rate for extra stochasticity time-series data within 100-steps, and showcasing a more unbaised eigenvalue spectrum of the fisher information matrix on CPU/GPU and IonQ QPU simulators.

==> sections/011_introduction.tex <==

Quantum machine learning (QML) holdexplores the potential of quantum computing to enhance the efficiency of training and evaluation, due to Quantum Circuit Simulation (QCS) directly models the mathematical structure of complex quantum states; after after announcing its annoucessupremacy against classical counterparts due to its unique probability-based characteristics \cite{b1}. The typical QML methods such as Quantum Neural Networks (QNNs) \cite{b2}, Variational Quantum Circuits (VQCs) \cite{b4}, Quantum Convolutional Neural Networks (QCNNs) \cite{cong2019quantum}, and Variational Quantum Linear Solver (VQLS) \cite{patil2022variational} speed up the training time and uncover the potential quantum calculation advantage, which accelerates the industrial applications, for instance, quantum deep learning \cite{wiebe2014quantum}, quantum thermal analysis \cite{webster2013nbsi}, and quantum heuristic transformer \cite{zhang2023transformer}. Even though these QML methods can tackle machine learning (ML) problems with tremendous speed-up, QML circuits could be verbosely deep and hard to simulate. In the current noisy intermediate-scale quantum (NISQ) era \cite{bharti2022noisy}, the HCQM learning methods proposed have proven successful in performing ML tasks (e.g., binary classification).

The typical QML methods such as Quantum Neural Networks (QNNs) \cite{b2}, Variational Quantum Circuits (VQCs) \cite{b4}, Quantum Convolutional Neural Networks (QCNNs) \cite{cong2019quantum}, and Variational Quantum Linear Solver (VQLS) \cite{patil2022variational} speed up the training time and uncover the potential quantum calculation advantage, which accelerates the industrial applications, for instance, quantum deep learning \cite{wiebe2014quantum}, quantum thermal analysis \cite{webster2013nbsi}, and quantum heuristic transformer \cite{zhang2023transformer}. Even though these QML methods can tackle machine learning (ML) problems with tremendous speed-up, QML circuits could be verbosely deep and hard to simulate. In the current noisy intermediate-scale quantum (NISQ) era \cite{bharti2022noisy}, the HCQM learning methods proposed have proven successful in performing ML tasks (e.g., binary classification).

Besides the circuit depth and inefficient simulation, the hybrid quantum model in quantum machine learning still faces many problems. For example, despite allowing thousands of unitary operations on IBM 128 qubits quantum photon chips - QPU, these devices are still unsuitable for training classical binary classification problems with shorter time and higher accuracy \cite{b5,b6}. In previous reviews, quantum algorithms revealed no exponential speed-up advantage due to limited qubits and quantum noises, especially when using real quantum hardware \cite{mcclean2018barren, montanaro2016quantum}. The HCQM highly relies on the number of qubits that quantum hardware provides since the computational graph within the quantum layer requires a high-precision quantum computer. While a Parameterized Quantum Circuit (PQC) offers trainable parameters akin to those in traditional neural networks, badly tuned unitary gates and exponential computation resources increase in RAM usage are impractical for real-world applications \cite{benedetti2019parameterized}. To tackle the problem effectively, HCQM is proposed. Some Quantum Transfer Learning (QTL) -based HCQMs are released \cite{transfer1, transfer2}, where the methods assume that pre-trained models can help quantum models to enhance the training efficiency. 

However, in scenarios where GPU and QPU resources are limited, a sequential HCQM (S-HCQM) cannot process classical data in separate stages and hardware. To characterize this phenomenon well, we propose a non-sequential HCQM (NS-HCQM) for executing classical machine learning binary classification tasks. To compare, recent studies \cite{arthur2022hybrid, chalumuri2021hybrid, hybird1, hybrid3} explored processing multiple classification problems but overlooked the non-sequential features of quantum models, as mentioned above. To elaborate, although the S-HCQM demonstrated high accuracy in classification tasks through modifying the pre-processing or post-processing layers of the HCQM, it failed to leverage the inherent multi-processing capabilities of the model. Similarly, Real-Amplitude N-Layer Quantum Networks \cite{kanno2021quantum} explored the potential of eliminating data re-uploading layers but overlooked the characteristic of multi-processing within the quantum model. In summary, the exploration of NS-HCQMs offers significant improvement in the training time and testing performance of quantum models in supervised image classification for NISQ devices. Nonetheless, prevailing studies in QML primarily address simplified scenarios \cite{s1, s2}, focusing on the sequential quantum processing by HCQMs and thus limiting their predictive probabilities and overall performance due to inherent challenges.

\textit{Challenge I}. How does the HCQM automatically calculate the long-distance gradients across the classic pre-trained model and the quantum-enhanced model (e.g. PQC)? To be more specific, The classical component handles tasks like data pre-processing and initial analysis, while the quantum component is used for processing complex patterns in the data that might be intractable for classical systems alone. Therefore, integrating classical and quantum parts in a single model requires a connection layer to optimize the whole system together, where the large computation cost within the middle layer becomes a widespread problem in HCQMs. Some existing studies \cite{qnn1, qnn2} try to capture the problem utilizing quantum-enhanced convolutional layers. The common problem is that a skyrocketing number of qubits is required as the higher resolution of images. Specifically, each convolutional block corresponds to one qubit, exacerbating the computational burden during gradient descent and rendering the training of HCQMs impractical.

\textit{Challenge II}. How to exploit the scalability of the HCQMs? As the complexity of HCQM grows, more and more RAM is required during the quantum simulation stage. Intuitively, we test HCQM on the quantum simulator before putting the model into a real QPU environment. In the quantum net of Fig. \ref{fig:hybrid}, the current quantum processors (NISQ devices) are limited in their number of qubits and are prone to errors. In other words, the less computing is required during the HCQM training part, the more scalability of the HCQM we can get. However, considering that using hundreds of logic qubits is nearly impossible, the core challenge here is how to improve the HCQM training robustness and efficient architecture for lower computing resources. By continuing, we notice that compact classical inputs help save the logical qubits but might negatively affect the core features. Therefore, based on these observations, there is a clear need for an innovative method that employs a parallel architecture to incorporate each node from the classical neural network. 




% \begin{figure*}[htbp]
% \centering
% \includegraphics[scale=0.35]{HQML.png}
% \caption{\label{fig:hybrid}The input features and pre-trained weights are integrated into the model. \(C_{in}\) denotes the classical inputs, where partial weights from the classical deep learning network are transferred to the quantum network. As depicted, each classical network corresponds to a quantum network, enabling high parallelism. After quantum processing, the output \(Q_{out}\) proceeds to the softmax layer. The parameters \(y_1\) and \(y_2\) represent the predicted labels \(C_{predict}\) for binary classification.}
% \end{figure*}

The strategies for the challenges mentioned above, we propose a novel model entitled Non-Sequential Hybrid Classic Quantum Model (NS-HCQM) consisting of two core modules: Hybrid Differentiable Optimization (HDO) and Parameterized Partial Entanglement Layer (PPEL). To solve \textit{Challenge I}, HDO is designed to optimize both classic unseen parameters and quantum trainable parameters. This is where the calculation of gradients and the use of back-propagation become essential. Due to the probabilistic foundation of quantum mechanics, contrasting with classical computing deterministic basis, calculating the long-distance computing gradients in a quantum system fundamentally differs from classical systems. Therefore, most existing studies capture this through the Parameter Shifting Rule (PSR) \cite{wierichs2022general} in the HCQM. That is to say, the gradient of the hybrid loss function undergoes standard back-propagation through the classical network. In the quantum segment, gradients are determined via the parameter shift rule and subsequently relayed to preceding classical layers. To solve \textit{Challenge II}, PPEL is proposed to process classical output non-sequentially so the quantum hybrid net can be separated into different blocks for seeking unique patterns of the problem dataset. Additionally, the quantum net can accept different features simultaneously so that the NS-HCQM largely improves the scalability. Specifically, within the non-sequential quantum network, decomposing tasks into smaller, shallow, and parallelizable units is a key strategy to reduce computation time and optimize resource allocation. Consequently, a dynamic resource can be allocated to each part of the NS-HCQM to exploit the unique features of the datasets and enhance the model performance}.

Last but not least, considering the sore point in the HCQM, i.e., lack of the efficient structure of the classical quantum connection layer, we additionally add the angle specified layer in our quantum embedding layer for optimization. To summarize, our main contributions are as follows:
\begin{itemize}
  \item We are the first to formulate the NS-HCQM in the classic binary classification realm regarding quantum machine learning (QML).
  \item Our novel methods related to NS-HCQM are proposed. To start with, the HDO provides our hybrid model with more capability to perform long-distance gradient calculation within hybrid nets. Secondly, we evaluate the result without components alongside with components, we conclude that our components can significantly increase the initial accuracy. In addition, utilizing local minima \cite{mcclean2018barren} instead of global alleviates the fluctuation during the quantum net training phase. To be precise, local cost can be updated more frequently than the global cost. In addition, the module PPEL can perform quantum weights training in different quantum simulators simultaneously.  
  \item Our extensive experiment is conducted utilizing the interface provided by Amazon Braket. We employ two publicly accessible datasets: Hymenoptera \cite{Walsh2021} and Brain Tumor \cite{Chaki2021}. The outcomes are demonstrated using our state-of-the-art model on the Amazon SV1 simulator and the Aria1 QPU.
\end{itemize} 

==> sections/022_results.tex <==
\section{Results}
In this section, we describe our simulation to test the NS-HCQM ability to handle classification tasks against the S-HCQM. We used Python and the Pennylane quantum simulation framework for development \cite{b3} and run hybrid job experiments on AWS Braket \cite{b47}. We start by explaining the dataset, benchmark, and model settings. Then, we discuss challenges like the barren plateau \cite{b49} and our optimization approach. We also include an ablation study and a comparison between NS-HCQM and S-HCQM. Results are detailed in the following subsections. The code used to produce the experiments is released on GitHub (anonymous).

\subsection{Datasets}\label{datasets}
We select two standard benchmark datasets and two image datasets (see Table \ref{tab:data}). The moon dataset comprises two interlocking half-circles that simulate the configuration of moons. In contrast, the spiral dataset has a coiled structure, which requires sophisticated non-linear decision boundaries. Furthermore, the Hymenoptera dataset contains a curated assemblage of annotated images depicting insects from the Hymenoptera order, including bees and ants, sourced from the homologous gene database. The Hymenoptera dataset is also introduced in CQNN \cite{mari2020transfer}. Apart from ad-hoc datasets, we choose the realistic Brain Tumor dataset, a comprehensive collection of magnetic resonance imaging (MRI) scans of annotated glioma and normal cases. In our case, we constrain our task to test the model performance on binary classification. For instance, we split the training part for S-HCQM and NS-HCQM. Finally, we test the one-hot encoding prediction on different datasets and hardware.

% NARMA10 involves 14 contributing terms, a 56\% increase from NARMA5's 9 terms, due to extended temporal dependencies and additional nonlinear interactions. Its memory dependency spans 12 time steps, 71\% more than NARMA5's 7 steps, requiring models to capture longer-term correlations effectively. Furthermore, NARMA10 introduces 83\% more nonlinearity, with 11 nonlinear terms compared to NARMA5's 6, amplifying the difficulty in disentangling input-output relationships. These factors highlight NARMA10's suitability for evaluating advanced models, particularly quantum neural networks (QNNs), which are designed to handle intricate dependencies and high-dimensional nonlinearities.

\begin{figure}
    \centering
    \begin{minipage}{0.55\textwidth}
        \centering
        \vspace{8pt}
        \adjustbox{max width=\linewidth}{
        \setlength{\tabcolsep}{6pt} % Default value: 6pt
        \def\arraystretch{1.7}%  1 is the default
        \begin{tabular}{ccccc}
         \thickhline
        \textbf{Id} & \textbf{Shape} & \textbf{Samples} & \textbf{Augmentation} \\ 
         \hline
        Moon &$2$ & $600$ &shuffle, noise \\ 
        Spiral & $2$ &$600$ &shuffle, turn \\
        Hymenoptera  & $224$ &$397$ &single crop, flip \\
        Brain Tumor & $224$ &$3625$ & single crop, flip\\
        \thickhline
        \end{tabular}
        }
        \vspace{10pt}
        \captionof{table}{The first two datasets are augmented by shuffle, noise, or turns. The Hymenoptera and Brain Tumor datasets contain flip and single crop, which entail the adjustment of the image data to a uniform length and differentiation.}
        \label{tab:data}
    \end{minipage}\hfill
    \begin{minipage}{0.43\textwidth}
        \centering
        \vspace{-5pt}
        \includegraphics[width=\linewidth]{anb.png}
        \includegraphics[width=\linewidth]{brain.png}
        \vspace{-18pt}
        \caption{Ants and bees dataset and brain tumor dataset.}
    \end{minipage}
\end{figure}


\begin{table}[h]

\label{Tbl:datasets}
\def\arraystretch{1.5}

\end{table}
\subsection{Experiment Settings}\label{e settings}

Experiments are conducted on the high-performance center (HPC) with one GPU node equipped with four NVIDIA CUDA 12.0 40 GB A100. For the NS-HCQM, we import the pre-trained ResNet18 from torchvision 0.17 and bridge the neural network with the proposed quantum net facilitated by Pytorch hybrid layers. The real hardware test utilizes the Amazon Pennylane plugin to connect the QPU.

\subsection{Model Settings}\label{p settings}
Initial hybrid model training experimentation was conducted to determine optimal hyperparameters for each model and dataset. To identify the hyperparameters for each model, we tend to use ad-hoc machine learning weights provided by \cite{eitrich2006efficient}. Therefore, we set \(\gamma\) to 0.1. The NN output shape is 512 for ResNet18. The pre-trained Image Net settings are version 1, which contains 1.2 million images that are categorized into 2 classes. The choice of loss functions Binary Cross-Entropy from logits was adopted for binary classification tasks. Moreover, in parallel settings, we specify that each quantum block, shown as one sphere in Fig. \ref{fig:hybrid}, utilizes two modules, HDO and PPEL. The details of quantum settings can be referred to Section \ref{models exp}. Regarding the output of logits, the scheduler decides when to drop the learning rate so the optimized cost gradually descends to a low point, and AAO modifies the circuit based on the cost weights. We select \(ReLU(x) = max(0, x)\) for non-linear activation and softmax function to predict the possibility of features.

\subsection{Main Results}
Before discussing our model results on real QPU with image datasets, we benchmark the model performance on the ad-hoc moon and spiral datasets. Several observations can be made from the figures: (1) The first moon benchmark evaluation showed that our model could achieve the perfect accuracy, as shown in Fig. \ref{Fig:moon} according to the model settings described in Section \ref{p settings}. The prediction of the spiral dataset illustrated in Fig. \ref{Fig:spiral} shows the good performance of our model in complex non-linear binary classification. In Table. \ref{tab:results}, the results demonstrate the HCQM models outperform the pure classical neural networks and NS-HCQM has the highest accuracy to fully exploit the classical features in the hybrid configuration. (2) Although S-HCQM achieves competitive results in classification tasks, NS-HCQM running time is still less than our proposed model. This is because we experimented on multiple simulators instead of feeding forward all the weights on a single quantum net. (3) Moreover, local simulations do not have any quantum hardware noise. Thus, the local simulated prediction accuracy is higher than Amazon-provided machines. (4) Both models can achieve promising results with shallow quantum circuit (i.e., the quantum circuit depth is less than or equal to ten.)


\begin{figure}[h]
\centering
\begin{minipage}{0.48\textwidth}
    \includegraphics[width=\linewidth]{moon_fit.png} 
    \captionof{figure}{Left image is the original moon dataset. The right image is the decision boundary of training after 100 epochs under the training of the NS-HCQM.}
    \label{Fig:moon}
\end{minipage}
\hspace{2pt} % Adjust this value to control the space
\begin{minipage}{0.48\textwidth}
    \includegraphics[width=\linewidth]{spiral fit.png}
    \setlength{\abovecaptionskip}{5pt}
    \captionof{figure}{Left image is the original spiral dataset. The right image is the decision boundary of training after 100 epochs under the training of the NS-HCQM.}
    \label{Fig:spiral}
\end{minipage}
\end{figure}

\begin{table}[t]
\centering
\caption{Benchmark on various binary classification tasks and average training time. (labeled with * results meaning hybrid classic model swapped the quantum part to a classic net)}
\label{tab:results}
\adjustbox{max width=\linewidth}{
\setlength{\tabcolsep}{8pt} % Default value: 6pt
\def\arraystretch{1.25}%  1 is the default
\begin{tabular}{cccccccccc}
\thickhline
\multirow{2}{*}{\textbf{Model}}  & 
\multicolumn{8}{c}{\textbf{Accuracy ($\uparrow$)}}  \\ \cline{2-10} &&
{\textbf{Moon}}                                                                & {\textbf{Spiral}}                                                              &                                                                     & {\textbf{Hymenoptera}}                                             &                                                           &                                                                     & {\textbf{Brain Tumor}}                                                  &                                                           \\ 
\midrule
HCM*  && 0.93                                                                & 0.90                                                                &                                                                 & 0.87                                                   &                                                      &                                                                 & 0.76                                                    &                                                       \\
\midrule
        &\begin{tabular}[c]{@{}c@{}}\textbf{Environment}\\ \textbf{Circuit}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Local\\ 10 qubits\end{tabular} & \begin{tabular}[c]{@{}c@{}}Local\\ 10 qubits\end{tabular} & \begin{tabular}[c]{@{}c@{}}Local\\ 10 qubits\end{tabular} & \begin{tabular}[c]{@{}c@{}}SV1\\ 34 qubits\end{tabular} & \begin{tabular}[c]{@{}c@{}}Aria1\\ 25 qubits\end{tabular} & \begin{tabular}[c]{@{}c@{}}Local\\ 10 qubits\end{tabular} & \begin{tabular}[c]{@{}c@{}}SV1\\ 34 qubits\end{tabular} & \begin{tabular}[c]{@{}c@{}}Aria1\\ 25 qubits\end{tabular} \\
        \cline{2-10} 
S-HCQM  &--& 0.97                                                                & 0.92                                                                & 0.89                                                                & 0.92                                                    & 0.91                                                      & 0.87                                                                & 0.78                                                    & 0.84                                                      \\
        && 8s                                                                  & 16s                                                                 & 18s                                                                 & 32s                                                     & 46s                                                       & 21s                                                                 & 46s                                                     & 48s                                                       \\

\textbf{NS-HCQM (Ours)} &--& \textbf{0.998}                                                               & \textbf{0.96}                                                                & \textbf{0.97}                                                                & 0.936                                                   & 0.92                                                      & \textbf{0.876}                                                               & 0.86                                                    & 0.88                                                      \\
        && 7s                                                                  & 16s                                                                 & 16s                                                                 & 31s                                                     & 38s                                                       & 18s                                                                 & 38s                                                     & 42s   \\
\thickhline
\end{tabular}%
}
\end{table}

We trained our model with 100 epochs and found that the NS-HCQM weight training can quickly reach nearly the highest accuracy. We also tested on the spiral benchmark dataset to demonstrate further our model in dealing with higher non-linearity datasets and, in comparison, noted that the inner circle of the spiral was misclassified in Fig. \ref{Fig:spiral}. 

Table. \ref{tab:results} presents evaluation results regarding hybrid and classic quantum models. Notably, hybrid classic quantum models outperform the classic model in binary classification tasks. This phenomenon is also consistent with previous findings\cite{s2}. Comparing S-HCQM and NS-HCQM, we conclude that the actual running time on Aria1 is longer than Amazon SV1 and local simulators, even though SV1 has 34 qubits. The result shows that NS-HCQM prediction accuracy significantly exceeds the hybrid classic model (HCM) and S-HCQM with less time consumption. 

\subsection{Ablation Study}
In this section, we conduct three ablation studies to evaluate the individual components of NS-HCQM performance. First, we evaluate the model without our proposed components, followed by an assessment with all components, and finally with the inclusion of the local minima which reduces the risk of the training staggering. Simply, we replace HDO and PPEL with standard gradient descent optimization and a single gate configuration. The results, shown in Fig. \ref{Fig:100bad}, demonstrate that omitting two proposed components allows the model to fit the data within 100 epochs but results in lower accuracy ($\sim$90\%). Furthermore, NS-HCQM with components largely improves the early-stage accuracy within the first five epochs. By contrast, when NS-HCQM is tested under identical conditions, Fig. \ref{Fig:100good1} without utilizing the local minima technique indicates it achieves near-perfect accuracy ($\sim$100\%) within a few epochs, despite some oscillation in the beginning, which proves our components viability.

\begin{figure}[H]
    \centering
    \begin{minipage}{0.3\textwidth}
        \centering
        \vspace{-5pt}
        \includegraphics[width=\linewidth]{plt3 (2).png}
        \vspace{-20pt}
        \captionof{figure}{Benchmark of NS-HCQM without components.}
        \label{Fig:100bad}
    \end{minipage}\hfill
    \begin{minipage}{0.3\textwidth}
        \centering
        \vspace{-5pt}
        \includegraphics[width=\linewidth]{plt1 (1).png}
        \vspace{-18pt}
        \captionof{figure}{Benchmark of NS-HCQM with components.}
        \label{Fig:100good1}
    \end{minipage}\hfill
    \begin{minipage}{0.3\textwidth}
        \centering
        \vspace{-5pt}
        \includegraphics[width=\linewidth]{plt2.png}
        \vspace{-18pt}
        \captionof{figure}{Benchmark of NS-HCQM with local minima.}
        \label{Fig:100good2}
    \end{minipage}
\end{figure}

As discussed in Section \ref{models exp}, we introduced a quantum dropout technique that partially connects the pre-trained weights to the quantum net to address the over-fitting issue. To reduce the potential barren plateau issue, the NS-HCQM only calculates the local minima as the local cost so each quantum block can use different parameter shifting. Eventually, the output is sent to the various nodes of the classical layer for optimization. The result of 100 epochs shown in Fig. \ref{Fig:100good2} verifies that adding the components vastly reduces the oscillation problem and alleviates the barren plateau problem. By looking at the period after only ten epochs, the learning curve still exists instead of gradients vanishing. Therefore, our proposed models are efficiently implementable for practical binary classification datasets.

% \begin{figure}[h]
% \def\arraystretch{1.5}
% \centering
% \includegraphics[width=0.45\textwidth]{100 epochs - seq.png} 
% \caption{The training and testing accuracy of the sequential hybrid quantum model in 100 epochs for 600 samples of the spiral dataset. The training accuracy starts at 50 \% and ends up at over 91 \%. There are no shows of over-fitting issues under 100 epochs.}
% \label{Fig:100seq}
% \end{figure}

% \subsection{Barren plateau and jax optimization}
% With the increasing number of quantum net layers and training epochs, the training part is more challenging to get the lowest energy since barren plateaus constitute a significant challenge in quantum machine learning \cite{b49}, as they can prevent optimization algorithms from fine-tuning hybrid model. This issue arises due to the random initialization of parameters in high-dimensional spaces, where it becomes increasingly likely for the optimizer to get stuck in a plateau at the start of training. Global cost functions, such as the expectation value of a system Hamiltonian, lead to barren plateaus even in shallow circuits due to the exponential scaling of the variance of the cost function gradient concerning the system size \((Var(\partial C/\partial \theta) \propto \exp(-n))\). This results in gradients that vanish exponentially. Conversely, employing local cost functions, which rely on local observables, modifies the gradient scaling to a polynomial rate. Our reliance on shallow circuits using local minima speeds up the training progress. Therefore, we sum our quantum net probability and distribute it to each wire evenly. 

% Besides, Grant et al. \cite{b52} addressed randomly chosen weights that might benefit the initial training steps. In gradients calculation, due to the exponential cache increase after each Jacobian matrix is calculated, the explosion number of each circuit affects the further parameters shifting. Our hybrid model only takes advantage of local minima instead of global calculation, which decreases the calculation intensity problem. Therefore, it is important to combine the pre-trained model into a quantum net since each training step is based on different calculations.

==> sections/033_discussion.tex <==
\section{Discussion}
In this paper, we develop a novel non-sequential hybrid classic quantum model designed to optimize the performance of image classification tasks within the constraints of the NISQ devices, which surpasses the sequential counterpart. Furthermore, we reveal that our model with local minima mitigates the training fluctuation problem. By leveraging a combination of quantum transfer learning, shallow parameterized quantum circuits, and an innovative embedding technique, our model demonstrates significant improvements in accuracy and efficiency over full-fledged sequential quantum hybrid models. Through reviewing \cite{b34}, we realize the limitation of computing resources. Our experimental results, validated on both simulated datasets and real quantum hardware, underscore the potential of our approach to utilize fewer qubits and computing resources while achieving higher accuracy. Meanwhile, we are aware that although simulating these hybrid quantum jobs on real QPUs indeed achieves promising results, the connection between quantum hardware and neural network interfaces still needs tunable parameters for further optimization.

Besides, we have presented the results of image classification tasks, and by comparing the classical layer case to the quantum layer case, we can show that NS-HCQM can achieve the quantum advantage. The core building block bridges the classic neural network outputs and quantum layers input. Although sequential hybrid quantum models can perform classification tasks with high accuracy, our more flexible NS-HQCM may takes advantage of future quantum-inspired computers that require QPU and GPU parallel training. In addition, there is a potential way to alleviate the oscillation during the hybrid model training by using disjoint parameter shift rules and the quantum dropout layer. Correspondingly, a quantum-processed dataset such as MINSQ \cite{b50} can accelerate convergence speed. Of course, the setup needs a more curated connection layer between classical and quantum neural networks and potentially more computing resources.

However, beyond the scope of our work, we notice that there are still challenges within the quantum machine learning realm. For instance, if the hybrid quantum model always proves to have a quantum advantage compared to its classical counterparts? How many layers in the hybrid model are considered a shallow hybrid model? Do the quantum encoder and decoder perform better than transformer-based pre-trained neural networks? What are the minimum quantum qubits to achieve high accuracy in deep learning tasks? Solving these still-existing problems will also raise some interesting questions regarding hybrid quantum models. In the future, we note that GPU-accelerated quantum methods might be an efficient way to improve both the performance and training time of the quantum machine learning model. 

==> sections/044_methods.tex <==
\section{Methods}
This section discusses the model structure and the main idea of connecting the classic model with the quantum model, taking advantage of pre-trained networks and quantum-enhanced features. We also introduce the two modules, HDO and PPEL. Then, we have a brief overview of the prediction net of the NS-HCQM. As we discussed before, our primary job is to find the optimized model layout for classification tasks.

\subsection{Model Overview}\label{models exp}

Here we first give an overview of HCQMs of non-sequential and sequential versions in Fig. \ref{Fig:seq_model} and Fig. \ref{Fig:nsq_model}. The optimized parameters transfer to a quantum support layer known as the quantum embedding layer from the feed-forward neural network, mapping the classical outputs into a quantum feature map. Additionally, We consider a classical N-dimensional data point x to be transformed into the phase of an n-qubit quantum state \(\ket{\psi_x}\). The quantum torch layer (torch layer implemented in a quantum circuit) in both graphs consists of different parameterized quantum gates defined by unitary operation. Each quantum gate contains fine-tuned weight w, angle a, and other coefficients that parameterize the gate effect, such as rotation angles around three axes (x, y, and z) referring to the "Rot" single arbitrary rotation gate in Fig. \ref{Fig:seq_model} and Fig. \ref{Fig:nsq_model}. In the quantum layer, all calculations are based on linear transformation. Therefore, the non-linear activation function serves in the prediction net. The significant difference between the NS-HCQM and S-HCQM is that in NS-HCQM, the non-sequential quantum layer can accept different node outputs parallelly, while in S-HCQM, the data flows into a sequential quantum layer directly.

\begin{figure}[h]
\def\arraystretch{1.5}
\centering
\includesvg[width=0.8\textwidth]{detailed1.svg} 
\caption{Sequential Hybrid Classic Quantum Model Structure.}
\label{Fig:seq_model}
\end{figure}

\begin{figure}[h]
\def\arraystretch{1.4}
\centering
\includesvg[width=0.8\textwidth]{detailed2.svg} 
\caption{Non-Sequential Hybrid Classic Quantum Model Structure with HDO.}
\label{Fig:nsq_model}
\end{figure}

The proposed model consists of two core modules, HDO and PPEL, which aim to capture long-distance optimization and improve model prediction accuracy. To be more specific, quantum differentiable parameters were updated linearly, and the efficiency depends on the simulation differentiation methods. In module HDO, the classical optimization function links the hybrid interface, and then the embedding layers are fed into the quantum net, where the optimization function can calculate the gradients within the HCQM. In this scenario, the module PPEL serves as a NN-like (neural network) net. To further capture the dataset features, the PPEL not only utilizes the correlated quantum gates regarding to embedding layer but includes partial entanglement connecting different qubits. PPEL can perform the classification tasks based on the previous weights and calculate the entangled weights to alleviate the overfitting problem. Additionally, inspired by the residual network, we pass one-third of pre-trained weights respectively to each input of arbitrary rotation gate (three-axis rotation gate) to reduce the computation intensity. Lastly, after the measurement, the quantum net selects the highest probability output to the prediction net. In the following, we will discuss the details of the two modules and prediction net. 

\subsection{Hybrid Differentiable Optimization}
The HDO module captures the parameter shifting during the HQCM training and updates the trainable parameters. In a classical neural network, the optimization carries the weights directly through the node connection. In this subsection, we first outline the Hadamard Dressing Wrap (HDW) serving as the initialization for the ansatz. Then, the following Y Angle Embedding Layer (Y-AEL) and Angle Adaptive Optimizer (AAO) present how to combine the classical and quantum optimization, calculating the largest gradients based on the specified quantum gate set.    

\subsubsection{Hadamard Dressing Wrap}
In our optimization structure, the HDW serves as the core part of the pre-processing quantum net. To solve \textit{Challenge I}, firstly, HDW distributes the quantum states into equal superposition probabilities. Specifically, quantum computing is based on undefined probability, and its classical counterpart renders defined outcomes. Despite directly mapping classical inputs to quantum feature maps that can achieve high quantum fidelity, the rendered quantum states lack classical core features. In other words, the extracted features might lose some accuracy after the transformation. Secondly, due to the equal probability characteristic of Hadamard transformation, the outcome is indecisive. Finally, the indecisive probability of each input will be distributed back to a decisive position with one Hadamard layer. Hence, we choose to wrap the full-fledged pre-processing quantum net with HDW for PPEL. 

\subsubsection{Angle Embedding Layer}
As discussed by embedding methods, the embedding function aims to minimize the loss of gradients calculation. In Hibert space, the distance between each two qubits is different. Hence, the parameters of the embedding are separable after the training. In Fig. \ref{Fig:model_details}, there are two blocks of Y-AEL encoding classical data into quantum systems via passing the classical parameters as the rotational angles of quantum gates. Besides, the effectiveness of the Y-AEL method depends on the invariability of \(R_y\). In other words, \(R_y\) embedding tunes the walking direction of each node in Hibert space. In the third subsection, we will discuss the correlation between Y-AEL and AAO.

\begin{figure*}[t]
\centering
\includegraphics[width=0.96\textwidth]{structure4.png} 
\caption{The full quantum circuit architectures with a symmetrical embedding layer and PPEL. The first layer is connected to each input with the Hadamard layer to distribute qubits into an unbiased superposition. The second part consists of one layer of Y Angle Embedding. The last layer returns the qubits to a differentiable probability using the Hadamard layer. Before the final expectation measurement layer, we choose arbitrary gates (three-axis rotation gates) and controlled rotation gates to change each qubit angle. The last axillary measured qubit (number 11) can conditionally adjust the entanglement block.}
\label{Fig:model_details}
\end{figure*}

\subsubsection{Angle Adaptive Optimizer}
Intuitively, the optimizer inside the HCQM is correlated to the previous embeddings, which share the same weights calculated by the quantum gates. Harper et al. demonstrate the efficiency of the adaptive optimizer in quantum optimization \cite{grimsley2019adaptive}. To simplify, we create a group of Y-angle and Z-angle specified controlled gates used for quantum optimization, which can be adaptively added to the quantum circuit with the loss of training changed by measuring the last auxiliary qubit. Consider a quantum system where the goal is to minimize a cost function \( C(\vec{\theta}) \), which could represent, for instance, the expectation value of a Hamiltonian \( H \) corresponding to the quantum circuit (QC). The cost function is dependent on the parameters \( \vec{\theta} = (\theta_1, \theta_2, \ldots, \theta_n) \) of the QC. The first step is to construct a parametric quantum circuit \( U(\vec{\theta}) \) with a set of gates \( \{G_i(\theta_i)\} \) selected from a predefined library. In our scenarios, \( \{G_i(\theta_i)\} \) refers to \(R_y\). The gradient of the cost function with respect to each gate parameter is computed. From the computed gradients, the gate \( G_j \) with the parameter \( \theta_j \) that has the largest absolute gradient is identified, which indicates that \( \theta_j \) has the most significant impact on the cost function at this step. That is to say, optimizing \( \theta_j \) could lead to a substantial decrease. After optimizing \( \theta_j \) for gate \( G_j \), the algorithm reassesses the circuit and repeats the gradient computation, gate supplement, and parameter optimization steps. 

\subsection{Parameterized Partial Entanglement Layer}
The module PPEL is proposed to classify the quantum data and reduce the computational resources that contain both single and entanglement gates as shown in Fig. \ref{Fig:model_details}, with each qubit connected to the next qubit with a non-local gate followed by two controlled rotation gate and two three-axis rotation local gates. To be precise, we use circular composed non-local entanglement gates to fully connect each qubit. In addition, a cost-benefit analysis \cite{McArdle_2022} reveals that the additional quantum resources required to implement an entangled layer are justified by a disproportionate increase in computational capabilities, thereby validating the layer efficiency from a resource-theoretical perspective. Except for the demonstrated 10 qubits, we incorporate two additional qubits for conditional measurement, increasing the flexibility of PPEL by enabling mid-circuit measurement adjustments during the training phase. In our study, PPEL demonstrates faster convergence towards the minimum energy state, thereby reducing the computational time.

To facilitate classification tasks, we propose the PQC with a partial entangled layer characterized by multi-qubit gates like controlled Y rotation gates and parameterized arbitrary two-qubit gates, significantly improving the final classification precision. Furthermore, the ability of the entanglement layer to generate more complex superposition and entanglement patterns allows a more accurate approximation of the fitting wave function than circuits with weak or no entanglement. To follow the same pattern of dense classical neural networks, we connect each data qubit (the qubits connected to the classical layer) to the ancilla qubit (the qubit utilized for mid-measurement). Specifically, we implement a strategy where each qubit is subject to a set of single quantum gates and entanglement gates, with the mid-measurement to condition the optimization. In the single gate specification, for instance, the PQC chooses to equip ten three-axis rotation gates maximumly which is consistent with the number of qubits. The integration of PPEL is presented in Algorithm \ref{alg}.

\begin{algorithm}
\caption{Intergration of PPEL}\label{alg}
\begin{algorithmic}[1]

\State Initialize quantum circuit with $N$ qubits
\State Prepare initial state $\psi_0$ using single-qubit rotation gates $R_y(\theta)$, $R_3(\phi, \theta, \omega)$, and HDW.

\Comment{Construct PPEL}
\For{$layer = 1$ \textbf{to} $L$ \textbf{step} $3$}
    \State set FLAG
    \If{$FLAG = 0$}
        \For{each pair of qubits $(i, j)$}
            \State Apply CNot gate to entangle $i$ and $j$
        \EndFor
        
    \ElsIf{$FLAG = 1$}
        \For{each pair of qubits $(i, j)$}
            \State Apply CRY gate or CYZ gate to entangle $i$ and $j$
        \EndFor
        
    \Else
        \For{each qubit $k$}
            \State Apply parameterized arbitrary rotation $R_{rot}(\phi, \theta, \omega)$
        \EndFor
    \EndIf
\EndFor

\State Measure the circuit to obtain output state $\psi_{\text{out}}$

\Comment{Optimization Loop}
\While{not converged}
    \State Compute the cost function $C = \langle\psi_{\text{out}}|H|\psi_{\text{out}}\rangle$
    \State Calculate gradients $\nabla C$ with respect to parameters $\{\theta, \phi\}$
    \State Update parameters using optimizer (e.g., gradient descent)
    \State Update the circuit with new parameters
    \State Measure the circuit to obtain new $\psi_{\text{out}}$
    \State Check convergence criterion (e.g., change in $C$ is below threshold)
\EndWhile

\State \textbf{return} Optimized parameters and classification accuracy
\end{algorithmic}
\end{algorithm}

\subsection{Prediction Net}
Finally, the prediction net of NS-HCQM refers to a post-processing quantum net with the softmax function to produce the output. Detailedly, The measurement quantum layer decodes the outcomes of quantum measurements into classical data, subsequently facilitating the derivation through the classical neural network. Furthermore, the prediction net operationalizes the conversion of quantum measurement outcomes, represented as a set of bitstrings \(\{b_1, b_2, \ldots, b_n\}\), into a normalized feature vector \(X\) suitable for classical processing. This process contains three primary stages:

\begin{enumerate}
    \item The quantum system, upon measurement, collapses into classical bitstrings with probabilities \(P(b_i)\), where \(i\) indexes the possible outcomes. The aggregation of these measurements can be formalized as the expectation value of an observable \(O\), calculated as:
   \begin{equation}
    \langle O \rangle = \sum_i P(b_i) O(b_i),   
   \end{equation}
   where \(O(b_i)\) denotes the value of the observable for the outcome \(b_i\).
   \item The aggregated data is then subject to normalization and feature extraction, yielding a feature vector \(X\). This process can be formalized as a mapping \(f: \langle O \rangle \mapsto X\), where \(X\) is designed to capture the essence of the quantum data in a format conducive to classical predictive models.
   \item The feature vector \(X\) serves as input to a classical model \(M\), with the predictive output \(y\) given by \(y = M(X)\). The choice of \(M\) and its parameters \(\theta\) are optimized to maximize the prediction accuracy.
\end{enumerate}
In our prediction net settings, the model calculates the cross-entropy loss of real and incorrect labels and utilizes AAO to perform the backpropagation.

==> sections/066_related_work.tex <==
\section{Related Work}
\subsection{Hybrid Quantum Computing}
The concept of Hybrid Quantum Computing (HQC) has developed gradually in the last two decades. Converting classical information into quantum units has been investigated in contemporary research to improve the processing of fixed datasets by quantum models \cite{lloyd2014quantum, rebentrost2014quantum}. Therefore, the pre-trained models can be regarded as the classical opponent of the whole hybrid model. Despite the efficiency of convolutional neural networks (CNNs) like AlexNet \cite{b35}, VGGNet \cite{b36}, ResNet \cite{b37}, and Inception(Google Net) \cite{b38} in image classification through rapid gradient descent calculation, their susceptibility to overfitting raises concerns about model generalizability. Hybrid Quantum Models (HQMs) emerge as potent feature extractors, unveiling novel features to improve generalization capability. Innovations in shallow quantum circuits and circuit sewing techniques have shown promising results \cite{b7}. Essential to NISQ device utilization, PQC via Variational Quantum Compiling (VQC) facilitates machine learning by enabling high-dimensional parallel computation through qubit superposition and entanglement \cite{b10, b11}. The hybrid approach merges the advantages of classical CNNs with quantum computing, extending learning capabilities into the NISQ era and beyond \cite{b34}.

Although Akinyemi et al. \cite{b30} demonstrate the powerfulness of tackling classical problems over traditional machine learning on small-scaled quantum models, it is significant for us to find generic efficient and highly transferable solutions for valuable tasks such as classification or regression problems \cite{b8}. Apart from the aforementioned models, Aijuan Wang et al. proposed a shallow HCQM \cite{hybird1}, which was able to process image classification. \cite{hybrid2} utilized the HCQM to solve short-term forecasting tasks.

\subsection{Quantum Machine Learning}
Recent advancements in quantum-driven machine learning algorithms have demonstrated superior efficiency over traditional methods for classical data tasks \cite{b12, rebentrost2014quantum}. These developments are supported by platforms that allow for the simulation or execution of quantum algorithms on cloud-based quantum devices \cite{b3}. Quantum phase estimation (QPE) algorithm \cite{dorner2009optimal} facilitates Quantum Fourier Transform \cite{QFT} to be performed on a quantum computer. Therefore, in quantum machine learning, the data can be efficiently mapped to a quantum feature map. Quantum Approximate Optimization Algorithm (QAOA) with QPE provides insights into adiabatic evolution on Hamiltonians, which can significantly help reduce the computational resources \cite{b21}. \cite{b22} analyzes the computational resources requirement indicating the risk of non-exponential acceleration advantage. A generic quantum machine learning circuit design relevant to these methods is detailed in \cite{b26}. Apart from the generic quantum machine learning method, Maria et al. find an efficient way to perform quantum machine learning tasks in limited Hilbert space \cite{schuld2019quantum}, providing the mathematical foundation for future quantum model training. In our research, we integrate a quantum machine learning hybrid approach with conventional machine learning tasks, leveraging insights from quantum transfer learning and pre-trained models.


==> sections/abstract.tex <==
\begin{abstract}
Quantum Machine Learning (QML) has emerged as an innovative framework with the potential to uncover complex patterns by leveraging quantum systems' ability to simulate and exploit high-dimensional latent spaces, particularly in learning tasks. We introduce \qp, a new non-sequential hybrid classical-quantum model architecture, leveraging quantum transfer learning, which enables efficient pattern recognition and temporal series data prediction by utilizing non-local parameterized quantum gates to enhance performance. Given the sensitivity of Quantum Neural Network (QNN) frameworks to gradient calculations and the computational capabilities of quantum hardware, we propose a mid-measurement circuit formalism with controlled and arbitrary rotation gates. Additionally, we develop a dynamic gradient selection method that applies the parameter shift rule on Quantum Processing Units (QPUs) and adjoint differentiation on GPUs. 
\qp\ incorporates variational quantum circuits (VQCs), dynamically exchanging the quantum information with the pre-trained weights from the classic model. Our results demonstrate model performance s exhibiting over 99\% accuracy in ad-hoc benchmarks, 100-step time-series prediction, and the broaden eigenvalue spectrum of fisher information matrix. Our result shows \qp\ enables 30x fast gradient learning and alleviates fluctuation in noisy density matrix quantum simulators and IonQ QPU. 
\end{abstract}


on both AMD Milan processor CPU and four A100 GPU
\begin{IEEEkeywords}
quantum machine learning, parameterized quantum circuit, quantum embedding, hybrid quantum model
\end{IEEEkeywords}

==> sections/abstract_v2.tex <==
\begin{abstract}
Quantum machine learning (QML) has emerged as an innovative framework with the potential to uncover complex patterns by leveraging quantum systems' ability to simulate and exploit high-dimensional latent spaces, particularly in learning tasks. We introduce quantum parallel information exchange (\qp) hybrid network, a new non-sequential hybrid classical quantum model architecture, leveraging quantum transfer learning, which enables efficient pattern recognition and temporal series data prediction by utilizing non-local parameterized quantum gates to enhance performance. Given the sensitivity of Quantum Neural Network (QNN) frameworks to gradient calculations and the computational capabilities of quantum hardware, we propose a mid-measurement circuit formalism with controlled and arbitrary rotation gates. Additionally, we develop a dynamic gradient selection method that applies the parameter shift rule on Quantum Processing Units (QPUs) and adjoint differentiation on GPUs. 
\qp\ incorporates variational quantum circuits (VQCs), dynamically exchanging the quantum information with the pre-trained weights from the classical model. Our results demonstrate model performance exhibiting over 99\% accuracy in ad-hoc benchmarks, lowering approximately 88\% convergence rate for extra stochasticity time-series data within 100-steps, and showcasing a more unbaised eigenvalue spectrum of the fisher information matrix on CPU/GPU and IonQ QPU simulators. Furthermore, our study shows that \qp\ enables 30-times faster gradient learning and alleviates fluctuation in noisy quantum simulators.
\end{abstract}

\begin{IEEEkeywords}
quantum machine learning, parameterized quantum circuit, quantum embedding, hybrid quantum model
\end{IEEEkeywords}
